Tensor Random Projection for Low Memory Dimension Reduction

Random projections reduce the dimension of a set of vectors while preserving structural information, such as distances between vectors in the set. This paper proposes a novel use of row-product random matrices in random projection, where we call it Tensor Random Projection (TRP). It requires substantially less memory than existing dimension reduction maps. The TRP map is formed as the Khatri-Rao product of several smaller random projections, and is compatible with any base random projection including sparse maps, which enable dimension reduction with very low query cost and no floating point operations. We also develop a reduced variance extension. We provide a theoretical analysis of the bias and variance of the TRP, and a non-asymptotic error analysis for a TRP composed of two smaller maps. Experiments on both synthetic and MNIST data show that our method performs as well as conventional methods with substantially less storage.

==> defs.tex <==
% Notes
\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{purple}{rgb}{0.3,0.0,.4}
\newcommand{\mnote}[1]{\textcolor{purple}{\textbf{[MU: #1]}}}
\newcommand{\lnote}[1]{\textcolor{blue}{\textbf{[LD: #1]}}}
% for restatement of lemmas and theorems
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{hyperref}
\usepackage{cleveref}
\RequirePackage{amsthm,amsmath}


\declaretheorem[name=Theorem,numberwithin=section]{thm}
% some traditional defintions that can be blamed on craig barratt
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}

\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}

\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bbm}{\begin{bmatrix}}
\newcommand{\ebm}{\end{bmatrix}}

% text abbrevs
\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}

\newcommand{\ones}{\mathbf 1}

% std math stuff
\newcommand{\reals}{{\mbox{\bf R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\eqbydef}{\mathrel{\stackrel{\Delta}{=}}}
\newcommand{\complex}{{\mbox{\bf C}}}
\newcommand{\sym}{{\mbox{\bf S}}}  % symmetric matrices

% lin alg stuff 
\newcommand{\Span}{\mbox{\textrm{span}}}
\newcommand{\range}{\mbox{\textrm{range}}}
\newcommand{\rank}{\mbox{\textrm{Rank}}}
\newcommand{\Rank}{\mbox{\textrm{Rank}}}
\newcommand{\nullspace}{{\mathcal {\bf nullspace}}}
\newcommand{\tr}{\mathop{\bf tr}}
\newcommand{\Tr}{\mathop{\bf tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{\lambda_{\rm min}}
\newcommand{\ms}{\mathop{\bf MaxSingVec}}
% probability stuff
\newcommand{\Expect}{\mathop{\bf E{}}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\erf}{\mathop{\bf erf}}
\newcommand{\sign}{\mathop{\bf sign}}

% convexity & optimization stuff
\newcommand{\Co}{{\mathop {\bf Co}}}
\newcommand{\co}{{\mathop {\bf Co}}}
\newcommand{\Var}{\mathop{\bf var{}}}
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\Ltwo}{{\bf L}_2}
%\renewcommand{\QED}{~~\rule[-1pt]{8pt}{8pt}}\def\qed{\QED}
\newcommand{\approxleq}{\mathrel{\smash{\makebox[0pt][l]{\raisebox{-3.4pt}{\small$\sim$}}}{\raisebox{1.1pt}{$<$}}}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\epi}{\mathop{\bf epi}}
%\newcommand{\hypo}{\mathop{\bf hypo}}
\newcommand{\var}{\mathop{\bf var}}
\newcommand{\Card}{\mathop{\bf card}}
\newcommand{\vol}{\mathop{\bf vol}}
\newcommand{\card}{\mathop{\bf card}}
\newcommand{\conv}{\mathop{\bf conv}}
\newcommand{\dom}{\mathop{\bf dom}}
\newcommand{\aff}{\mathop{\bf aff}}
\newcommand{\cl}{\mathop{\bf cl}}
\newcommand{\Angle}{\mathop{\bf angle}}
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\relint}{\mathop{\bf rel int}}
\newcommand{\bd}{\mathop{\bf bd}}
\newcommand{\vect}{\mathop{\bf vec}}
\newcommand{\dsp}{\displaystyle}
\newcommand{\foequal}{\simeq}
\newcommand{\VOL}{{\mbox{\bf vol}}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\xopt}{x^{\rm opt}}
\newcommand{\prox}{{\bf prox}}
\newcommand{\conj}{{\bf conj}}
\newcommand{\update}{\mathop{\bf update}}
\newcommand{\indicator}{{\bf 1}}

% for statistics
\newcommand{\huber}{\mathop{\bf huber}}
\newcommand{\sort}{\mathop{\bf sort}}
\newcommand{\round}{\mathop{\bf round}}


% for prettiness
\newcommand{\half}{(1/2)}

% for constants 
\newcommand{\constanta}{\frac{\sigma_{\min}(\mathcal{A}_{V^\star})}{4\|\mathcal{A}\|_{op}}}
\newcommand{\constantb}{\frac{2\cdot \constanta \lambda_{\min>0}(Z^\star)}{4\frac{1}{\sigma_{\min}(\mathcal{D})}\sqrt{1+4\cdot \constanta}+1}}
\newcommand{\constantc}{\frac{2\cdot \constantb\lambda_{\min>0}(X^\star)}{\sqrt{4\|Z^\star\|_{op}+4\constantb}+4\|Z^\star\|_{op}}} 
\newcommand{\constantd}{\frac{\lambda^2_{n-r}(Z^\star)}{\frac{1}{\sigma^2_{\min}(\mathcal{D})}(4\sqrt{\|Z^\star\|_{op}}+2\sqrt{ \frac{\lambda_{n-r}(Z^\star)}{\frac{1}{\sigma_{\min}(\mathcal{D})}}})^2}\lambda_{\min >0}(X^\star)}
\newcommand{\constante}{ \frac{\lambda_{\min>0}(X^\star)\|Z^\star\|_{op}}{10(\frac{1}{\sigma_{\min}(\mathcal{D})}+\frac{1}{\sigma^2_{\min}(\mathcal{D})}}}
\newcommand{\constantA}{\frac{\|\mathcal{A}(VSV^\top)-b\|}{\sigma_{\min}(\mathcal{A}_V)} +\|S\|_{op}}
\newcommand{\constantD}{(1+\kappa)\frac{\epsilon}{T}}
\newcommand{\constantE}{(1+\kappa)\sqrt{\frac{\epsilon}{T}}}
\newcommand{\constantB}{\frac{1}{4}\biggr[ \sqrt{(\constantE)^2+4[\constantA] +4\constantD}+\constantE\biggr]^2}

% theorems
%\theoremstyle{definition} % don't italicize theorems
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}

% alg description --- not much for now!
\newenvironment{algdesc}%
{\begin{quote}}{\end{quote}}

% figures
\def\figbox#1{\framebox[\hsize]{\hfil\parbox{0.9\hsize}{#1}}}
% figure size
\makeatletter
\newlength \figwidth
\if@twocolumn
  \setlength \figwidth {0.9\columnwidth}
\else
  \setlength \figwidth {0.5\textwidth}
\fi
\makeatother

% \showthe\figwidth

% captions a la sirev
\makeatletter
\long\def\@makecaption#1#2{
   \vskip 9pt
   \begin{small}
   \setbox\@tempboxa\hbox{{\bf #1:} #2}
   \ifdim \wd\@tempboxa > 5.5in
        \begin{center}
        \begin{minipage}[t]{5.5in}
        \addtolength{\baselineskip}{-0.95pt}
        {\bf #1:} #2 \par
        \addtolength{\baselineskip}{0.95pt}
        \end{minipage}
        \end{center}
   \else
	\hbox to\hsize{\hfil\box\@tempboxa\hfil}
   \fi
   \end{small}\par
}
\makeatother

==> structural-random-projection.tex <==
\section{Structured Random Mapping}
Given a large vector
We seek a random projection map to embed a collection of vectors
$\mathcal X \subseteq \mathbb{R}^{d}$
into $\mathbb{R}^k$ with $k \ll d$.
Let us take $d = \prod_{n=1}^N d_n$, motivated by the problem of compressing
(the vectorization of) an order $N$ tensor with dimensions $d_1,\ldots,d_N$.

Conventional random projections use $O(kd)$ random variables.
Generating so many random numbers is costly; and storing them can be costly when $d$ is large.
Is so much randomness truly necessary for a random projection map?

% Indeed, we show it is not.
To reduce the randomness and storage requirements for DRMs, we propose
the \emph{tensor random projection} (TRP):
\begin{equation}
\label{eq:TRP}
f_{\text{TRP}}(\mathbf{x}):= (\mathbf{A}_1 \odot \cdots \odot \mathbf{A}_N)^\top
\mathbf{x},
\end{equation}
where each $\mathbf{A}_i \in \mathbb{R}^{d_i \times k}$, for $i \in [N]$,
can be an arbitrary RP map and
$\mathbf{A} := (\mathbf{A}_1 \odot \cdots \odot \mathbf{A}_N)^\top$.
We call $N$ the \emph{order} of the TRP.
This construction is inspired by the CANDECOMP/PARAFAC (CP) decomposition in
low-rank tensor approximation \cite{kolda2009tensor}.
We show in this paper that the TRP is an expected isometry,
has vanishing variance,
and supports database-friendly operations.
%For more background knowledge about tensor decomposition, please refer to \cite{kolda2009tensor}.

The TRP requires only $k\sum_{i = 1}^N d_i$ random variables
(or $k\sqrt[N]{d}$ by choosing each $d_i$ to be equal),
rather than the $kd$ random variables needed by conventional methods.
Hence the TRP is database friendly:
it significantly reduces storage costs and randomness requirements compared to its
constituent DRMs.

In large scale database settings,
where computational efficiency is critial and queries of vector elements are expensive,
practitioners often use sparse RPs.
Let $\delta$ be the proportion of non-zero elements in the RP map $\mathbf{A}$.
To achieve a $\delta$-sparse RP, a common construction is the scaled sign random map:
each element is distributed as $(-1/\sqrt{\delta}, 0, 1/\sqrt{\delta})$ with probability
$(\delta/2, 1-\delta, \delta/2)$.
\cite{achlioptas2003database} proposed $\delta=1/3$,
while \cite{li2006very} further suggests a sparser scheme with
$\delta=1/\sqrt{d}$ that he calls the \textit{Very Sparse} RP.
Following this definition, we can form a TRP whose constituent submatrices
are generated each with sparsity factor $\delta$, which leads to a $\delta^N$-sparse TRP.
This TRP is highly database friendly: applying the map requires few queries and no floating point operation.
Below, we show this very sparse TRP also performs well (is a low-variance approximate isometry)
in theory and in practice.

\paragraph{Variance Reduction}
One quirk of many DRMs is that the variance of the map is controlled by the range $k$ of the map.
However, with the TRP we can reduce the variance without increasing $k$.
We propose the \emph{TRP(T)},
a scaled average of $T$ independent TRPs we call \emph{replicates},
defined as
\begin{equation}
f_{\text{TRP(T)}}(\mathbf{x}):= \frac{1}{\sqrt{T}}\sum_{t = 1}^T f^{(t)}_{\text{TRP} }(\mathbf{x}).
\end{equation}
(Notice that the average of $T$ TRPs is not itself a TRP; this property is unusual among RPs.)
We discuss its theoretical properties in the main theory section below.


==> theoretical_development.tex <==
\section{Main Theory}
In this section, we will show the TRP and TRP(T) are expected isometries with vanishing variance.
We provide a rate for the decrease in variance with $k$.
We also prove a non-asymptotic concentration bound on the quality of the isometry when $N=2$.
%but leave the task of building concentration bound for $N\ge 3$ case for the future exploration.
Without loss of generality, we state our results only for the TRP(T),
since the TRP follows as a special case with $T=1$.

We begin by showing the TRP is an approximate isometry.
\begin{lem}
\label{lemma: norm-preserve}
Form a TRP(T) %of order $N$ with range $k$
composed of independent matrices with independent isotropic columns.
%whose entries are mean zero, variance one, and within each column every pair of elements has covariance zero.
Then
\begin{equation}
\label{eq:lemma-invariant-length-statement}
\mathbb{E} \|f_{\textup{TRP(T)}}(\mathbf{x})\|^2 = \|\mathbf{x}\|^2. \nonumber
\end{equation}
\end{lem}
Interestingly, \cref{lemma: norm-preserve} does not require elements of $\mathbf{A}_n$ to be iid.

Now we present an explicit form for the variance of the isometry.
\begin{lem}
\label{lemma:variance}
Fix $\mathbf{x} \in \mathbb{R}^{\prod_{n=1}^N d_n}$.
Form a TRP(T) of order $N$ with range $k$
independent matrices whose entries are iid with
mean zero, variance one, and fourth moment $\Delta$.
Then
\begin{equation*}
% \begin{aligned}
% &\textrm{Var}(\|f_{\textup{TRP}}(\mathbf{x})\|^2) = \frac{1}{k}\left[ (\Delta^N-3)\|\mathbf{x}\|_4^4 +2\|\mathbf{x}\|_2^4\right] ,\\
% &\textrm{Var}(\|f_{\textup{TRP(T)}}(\mathbf{x})\|^2) = \frac{1}{Tk}(\Delta^N-3)\|\mathbf{x}\|_4^4 + \frac{2}{k}\|\mathbf{x}\|_2^4.
% \end{aligned}
% \var(\|f_{\textup{TRP}}(\mathbf{x})\|^2) = \frac{1}{k}(\Delta^N-3)\|\mathbf{x}\|_4^4 + \frac{2}{k}\|\mathbf{x}\|_2^4,
% \qquad
\var(\|f_{\textup{TRP(T)}}(\mathbf{x})\|^2) = \frac{1}{Tk}(\Delta^N-3)\|\mathbf{x}\|_4^4 + \frac{2}{k}\|\mathbf{x}\|_2^4.
\end{equation*}
\end{lem}
We can see the variance increases with $N$.
In the $N=1$ Gaussian case, this formula shows a variance of $2/k \|\mathbf{x}\|_2^4$,
which agrees with the classic result.
Notice the TRP(T) only reduces the first term in the variance bound:
as $T\rightarrow \infty$, the variance converges to that of a Gaussian random map.

Finally we show a non-asymptotic concentration bound for $N=2$.
We leave the parallel result for $N\ge 3$ open for future exploration.
\begin{prop}
	\label{prop: N-2-bound}
  Fix $\mathbf{x} \in \mathbb{R}^{d_1 d_2}$ with sub-Gaussian norm $\varphi_2$.
  Form a TRP(T) of order 2 with range $k$
  composed of two independent matrices whose entries are drawn iid
  from a sub-Gaussian distribution with mean zero and variance one.
  Then there exists a constant $C$ depending on $\varphi_2$
  and a universal constant $c_1$
  so that
	\begin{equation}
%	\begin{aligned}
	\label{eq:lemma-invariant-length-statement}
	\mathbb{P}\left(\left| \|f_{\text{TRP(T)}}(\mathbf{x})\|^2 - \|\mathbf{x}\|^2_2 \right| \ge \epsilon \|x\|^2\right)\le C\exp\left[ - c_1 \left(\sqrt{k}\epsilon\right)^{1/4} \right],\nonumber
%	\end{aligned}
	\end{equation}
	\mnote{Verify no dependence on $T$}
\end{prop}
Here $\varphi_2$ is the sub-Gaussian norm defined in \cref{def:sub-gaussian} in Appendix \ref{sec:appendix_proof}.
\cref{prop: N-2-bound} shows that for a TRP to form an $\epsilon$-JL DRM
with substantial probability on a dataset with $n$ points,
our method requires $k=\mathcal{O}(\epsilon^{-2}\log^8 n)$ while
conventional random projections requires $k=\mathcal{O}(\epsilon^{-2}\log n)$.
Numerical experiments suggest this bound is pessimistic.

